Estimating ionization states and continuum lowering from ab initio path integral Monte Carlo simulations for warm dense hydrogen

Warm dense matter (WDM) is an active field of research, with applications ranging from astrophysics to inertial confinement fusion. Ionization degree and continuum lowering are important quantities to understand how materials behave under these conditions, but can be difficult to diagnose since experimental campaigns are limited and often require model-dependent analysis. This is especially true for hydrogen, which has a comparably low scattering cross section, making high quality data particularly difficult to obtain. Consequently, building equation of state tables often relies on exact simulations in combination with untested approximations to extract properties from experiments. Here, we investigate an approach for extracting the ionization potential depression and ionization degree -- quantities which are otherwise not directly accessible from the physical model -- from exact ab initio path integral Monte Carlo (PIMC) simulations utilizing a chemical model. In contrast to experimental measurements, where noise and non-equilibrium effects add to the uncertainty of the inferred parameters, PIMC simulations provide a clean signal with well-defined thermodynamic conditions. Comparisons against commonly used models show a qualitative agreement, but we find deviations primarily for the high density and high temperature cases. We also demonstrate the decreasing sensitivity of the dynamic structure factor with respect to both ionization and continuum lowering for increasing scattering angles in x-ray Thomson scattering experiments. Our work has important implications for the design of future experiments, but also offers qualitative understanding of structure factors and the imaginary-time correlation function obtained from exact quantum Monte Carlo simulations.

==> notes.tex <==

\section{Hannah's Notes}

Please ignore... \smiley

\begin{enumerate}
    \item add chi as output for each optimisation
    \item Z-q-chi heatmap
        \begin{itemize}
            \item[-] see Fig. \ref{fig:surface-map-dataset3} and \ref{fig:log-surface-map-dataset3}
        \end{itemize}
    % \item (as in calculate chi over different Z for each q value)
    \item reproduce Fig. 1 in PhysRevLetter121 Dornheim 2018 to see stuff
    \item reproduce Fig. 2 here as a heatmap and chi for q and tau/beta
    \item optimize for all q at once
    \item use LFC and compare behaviour for different model options, this could be related to the point below
    \item look at q about 2 and WR where all three datasets seem to have something weird
    \item compute rayleigh weight for meaningful Z, IPD for each dataset using AR-XRTS (?)
    \item use FEOS, SESAME EoS models to compare against
\end{enumerate}


19.04.2024 Update meeting
\begin{enumerate}
    \item repeat process for different theta, rs values - Done
    % \item see point above: reproduce Fig. 1 in PhysRevLetter121 Dornheim 2018
    \item calculate ipd, Z from models (Stewart-Pyatt, Ecker Kroll) for const. theta and then const. rs - Done
    \item send Tobias WR values for best fit
    \item repeat runs for higher beam energy to get more angles from q-values (PIMC) - Done
    \item fit for all-q at once for each dataset and separately
    \item repeat fit for rs1, theta=1 and look at error distribution - Done
    \item calculate error distribution of mcss against pimc (see equation) for all q individually and all q combined
    \item put a measure on whether mcss can reproduce pimc and how tau, q dependent this is
    \item see point above: reproduce Fig. 1 in PhysRevLetter121 Dornheim 2018 for best fit
    \item leave ipd as a free parameter and produce a best fit
    \item increase beam energy to reduce the angles calculated from q - having some issues with this, cause it leads to huge runtimes 
\end{enumerate}

01.07.2024 Notes
\begin{enumerate}
    \item best fit algorithm seems to work as expected
    \item Repeat Fig. 11 for smaller step size between ionisation to find actual best Z and compare against best fit and previous fit
    \item We expect a good fit for small $q$ (this is where plasmon behaviour dominate and the Chihara decomposition makes the most sense), for medium $q$ exchange correlations dominate and we would not expect a decent fit, as Chihara decomposition is unable to capture the behaviour correctly
    \item Fig \ref{fig:best-fit-attempt-dataset3} gives an overview of the best fit outputs for dataset3, using the first 4 $q$-values only. This shows the expected best fit value at $Z=0.367$, which somewhat disagrees with the best fit for $q=0$ for the individual fit.
    \item This behaviour needs to be investigated further
    \item The tolerance for the individual fits could have been too high, to not give the actual minimum value (double check this)
\end{enumerate}

best fit = fit all q-values at once!!!



\subsection{Some equations}

MCSS requires several inputs, the important ones here are an input temperature (in units of $\unit{eV}$), mass density ($\rho$ in units of $\unit{g/cm^3}$) and angle ($\theta$ in degrees).
These are derived from the PIMC results for $q$, $r_s$ and $\Theta$ as:
\begin{equation*}
    \rho = \frac{3}{4 \pi (r_s a_0)^3} \frac{m_\text{atm}}{1000}
    \,,
\end{equation*}
\begin{equation*}
    T_e = \frac{E_F \Theta }{k_B}
    \,.
\end{equation*}
The small angle approximation is used here to calculate a value for the scattering angle from the PIMC $q$ inputs.
This is taken from the small angle approximation for the momentum shift variable $q$ (see Eqn. (9) in \cite{Dornheim_T_follow_up}).
\begin{equation*}
    \theta = \frac{180}{\pi} 2 \arcsin{\left[ \frac{\hbar c q}{2 E_0} \right]}
    \,.
\end{equation*}
Here, $a_0$ is the Bohr radius, $k_B$ is the Boltzmann constant, $\hbar$ is the Dirac constant (reduced Planck constant), $c$ is the speed of light, all in SI Units.
Note that the atomic mass $m_\text{atm}$ here is given in SI units (i.e. $\unit{kg}$).
The Fermi energy $E_F$ is calculated using:
\begin{equation*}
    E_F = \frac{\hbar^2}{2 m_e} \left( \cfrac{9 \pi}{4 (r_s a_0)^3} \right)^\frac{2}{3}
    \,.
\end{equation*}
All PIMC inputs are given in Hartree units.
MCSS takes mostly cgs/ SI inputs.
%, with the following conversion factors used:
% \begin{itemize}
%     \item J to eV: $\num{6.241509e18}$
%     \item K to eV: $\num{8.61732814974056E-05}$
%     \item Ha to eV: $\num{27.211386}$
% \end{itemize}
The Fermi-wavevector $q_F$ is defined as:
\begin{equation}
    q_F = \left(\frac{9 \pi}{4 r_s^3} \right)^{1/3}
\end{equation}

\begin{equation}
    r_s = \frac{1}{a_0} \left(\frac{3}{4 \pi n_e} \right)
\end{equation}

Also, from \cite{Dornheim_POP_2017} (note that there is a mistake in the expression for the plasma frequency following Eqn. (1), missing square-root):
\begin{equation}
    \omega_{pe} = \sqrt{\frac{e^2 n_e}{\epsilon_0 m_e}} \quad \Bigg(=\sqrt{\frac{3}{r_s^3}} \, \text{(in HAU)} \Bigg)
\end{equation}

\subsection{Initial Results}

Some initial results for the datasets (overview given in Table \ref{tab:dataset-overview}) for optimising the IPD and ionisation simultaneously are given below.
Since they are both inherently linked quantities, we decided to move forward by separating out and optimising for one or the other.
Results are shown in Figures \ref{fig:initial-results1}, \ref{fig:initial-results2}, \ref{fig:initial-results3}.
From these figures, it becomes obvious that the Laplace transform of the dynamic structure factor from MCSS has some asymmetry to it, and often predicts a slightly different temperature than the given input value.
To confirm this asymmetry of the structure factor in the Laplace transform giving different temperatures, the following equation was applied.
Following previous work, the temperature can be directly obtained from the ITCF, by finding the minimum in $\tau$ space corresponding to the temperature.
Using detailed balance, the temperature can be calculated from the free-free, bound-free and total components as:
\begin{equation*}
    T = \cfrac{\omega}{\log{\left[ \frac{S(-\omega)}{S(\omega)}\right] } }
\end{equation*}
We found however, that MCSS uses an additional term $\frac{w_s}{w_i}$ for the scattered and initial frequencies to 'normalise' the structure factor contributions.
The contribution of this normalisation factor can be observed in Fig \ref{fig:calculated-temperatures-mcss} and following, where including this factor has a clear impact on the output.
This does not however, solve the issue of why the temperature is not constant, or why the free-free and bound-free structure are so different in shape.
It does imply however, that there is some function, dependent on the frequency, that is used for normalisation of some kind in MCSS.
This function is however different for the free-free and bound-free components.
Not sure what's going on there...

\begin{table}
\begin{tabular}{l|c|c|c|c|c|c}
      & \textbf{$N$} & \textbf{\emph{$\Theta$}} & \textbf{\emph{$r_s$}} & \textbf{$\rho$} & \textbf{$T_e$} & \textbf{Status/ Notes} \\
     \hline
     1 & 14 & $1$ & $1$  & $2.70$ & $50.11$ &   Re-run at higher beam energy\\
     2 & 14 & $1$ & $2$ & $0.33$ & $12.53$ &  Re-run at higher beam energy\\
     3 & 14 & $1$ & $3.23$ & $0.08$ & $4.80$ &  Re-run at higher beam energy\\
     %
     4 & 14 & $1$ & $2.5$  & $0.17$ & $8.02$ & Re-run \\
     5 & 14 & $1$ & $2.75$  & $0.13$ & $6.63$ & Re-run \\
     6 & 14 & $1$ & $3.$  & $0.09$ & $5.57$ & Re-run \\
     %
     7 & 14 & $2$ & $3.23$  & $0.08$ & $9.61$ & Re-run \\
     %
     \hline
     8 & 32 & $1$ & $1.$  & $2.70$ & $50.11$ & Processed \\
     9 & 32 & $1$ & $2.$  &  $0.33$ & $12.53$ & Processed \\
     10 & 32 & $1$ & $3.23$  & $0.08$ & $4.80$ & Processed \\
     %
     11 & 32 & $2$ & $3.23$  & $0.08$ & $4.80$ & Processed \\
     12 & 32 & $4$ & $3.23$  & $0.08$ & $19.21$ & Processed \\
     13 & 32 & $8$ & $3.23$  & $0.08$ & $38.43$ & Processed \\
\end{tabular}
\caption{Overview of the PIMC and MCSS input values used to model each data set initially.}\label{tab:dataset-overview}
\end{table}


Turns out the issue lies in the approximation for $q$, which leads to some deviation for smaller beam energies (see Fig. \ref{fig:temperature-plots-for-increasing-beam-energies}).
While this approximation is usually assumed to be appropriate for XRTS, recent work has shown that it can lead to some deviation from the exact result.
MCSS does not properly account for this effect in XRTS mode, but does include the full effect for OTS.
Some modifications were made within MCSS to account for this discrepancy.
A dynamic structure factor fulfilling detailed balance can be achieved by fixing the approximate $q$-expression and removing the unnecessary $(w_s/w_i)^2$ factor.

\begin{figure*}
    \includegraphics[width=0.98\linewidth]{pics/old/1_result_index=0.png}
    \includegraphics[width=0.98\linewidth]{pics/old/1_result_index=6.png}
    \caption{Best fit for low (top) and high (bottom) q values for dataset 1, with $\rho=2.7 \unit{g/cm^{-3}}$ and $T=50 \unit{eV}.$}
    \label{fig:initial-results1}
\end{figure*}

\begin{figure*}
    \includegraphics[width=0.98\linewidth]{pics/old/2_result_index=0.png}
    \includegraphics[width=0.98\linewidth]{pics/old/2_result_index=28.png}
    \caption{Best fit for low (top) and high (bottom) q values for dataset 2, with $\rho=0.33 \unit{g/cm^{-3}}$ and $T=12.53 \unit{eV}.$}
    \label{fig:initial-results2}
\end{figure*}


\begin{figure*}
    \includegraphics[width=0.98\linewidth]{pics/old/3_result_index=0.png}
    \includegraphics[width=0.98\linewidth]{pics/old/3_result_index=28.png}
    \caption{Best fit for low (top) and high (bottom) q values for dataset 3, with $\rho=0.08 \unit{g/cm^{-3}}$ and $T=4.8 \unit{eV}.$}
    \label{fig:initial-results3}
\end{figure*}


\begin{figure*}
    \includegraphics[width=0.5\linewidth]{pics/old/1_result_index=0_temperature_calculated.png}
    \caption{
    Representation of detailed balance for the MCSS structure factor outputs for dataset 1 for $q=1.61724$.
    Left: The temperature calculated using detailed balance for each component of the structure factor from MCSS is plotted against $\omega$, the horizontal constants indicate the temperatures predicted by MCSS and Tobias' method.
    Right: The free-free and bound-free structure factors are plotted for the negative scattering range. New here refers to the components normalised by a factor of $(w_s/w_i)^{-1}$, as mentioned above, whereas old refers to the original outputs without the additional multiplier.
    }
    \label{fig:calculated-temperatures-mcss}
\end{figure*}


\begin{figure*}
    \includegraphics[width=0.5\linewidth]{pics/old/2_fixed_result_index=2_temperature_calculated.png}
    \caption{
    Representation of detailed balance for the MCSS structure factor outputs for dataset 2 for $1.40057$.
    Left: The temperature calculated using detailed balance for each component of the structure factor from MCSS is plotted against $\omega$, the horizontal constants indicate the temperatures predicted by MCSS and Tobias' method.
    Right: The free-free and bound-free structure factors are plotted for the negative scattering range. New here refers to the components normalised by a factor of $(w_s/w_i)^{-1}$, as mentioned above, whereas old refers to the original outputs without the additional multiplier.
    Detailed balance issues previously observed are fixed here.
    }
    \label{fig:calculated-temperatures-mcss-fixed}
\end{figure*}




\begin{figure*}
    \includegraphics[width=\linewidth]{pics/old/result_temperature_calculated_for_different_beam_energies.png}
    \caption{The same case as previously, for small q, where the beam energy is now increased to account for the irregularities. As observed, detailed balance is given for increasingly high beam energies.
    The cause was found to be the use of the approximation for $q$, leading to asymmetries in the ITCF for lower beam energies.}
    \label{fig:temperature-plots-for-increasing-beam-energies}
\end{figure*}


\subsubsection{Saha equation}


\begin{figure*}
    \includegraphics[width=\linewidth]{pics/old/ipd_output_plotted.png}
    \caption{
    Logarithmic plot of the Saha equation output against ionisation state $Z$.
    Black lines indicate the ''cut-off'' at the Hydrogen binding energy of $13.6 \unit{eV}$.
    }
    \label{fig:saha-output}
\end{figure*}

Since IPD and ionisation are inherently related, optimizing for both simultaneously could introduce overfitting.
Instead, the IPD can be directly calculated for a given ionization state using the Saha equation \cite{Saha_prs_1921}.
For a single-atom plasma, the equation reads:
\begin{equation}
    \frac{n_i}{n_{i+1}} = \frac{g_i}{g_{i+1}} \exp{ \left[ \beta \mu - \beta E_\text{i,eff} \right]}
    \,,
\end{equation}
for the population of the i-th ionization state $n_i$, the statistical weight $g_i = 2 \text{J}+1$, the chemical potential $\mu$ and the inverse temperature $\beta=\frac{1}{k_B T}$.
The effective binding energy $E_\text{i,eff}$ here is defined in terms of the actual binding energy for the 1s Hydrogen state $E_b = 13.6 \unit{eV}$ and the energy shift provided by the IPD (here $\Delta_\text{IPD}$) as
\begin{equation*}
    \beta E_\text{i,eff} = \beta(E_b - \Delta_\text{IPD})
    \,.
\end{equation*}
Thus, the IPD can be directly calculated from the ionization state as
\begin{equation}
    \Delta_\text{IPD} = E_b - \mu + k_B T \ln{ \left[\frac{g_{i+1}}{g_i} \frac{n_i}{n_{i+1}} \right]}
    \,.
\end{equation}
For a hydrogen atom, the ith state refers to the ground state, whereas i+1 indicates the excited Hydrogen atom.
Note that only excitation from the 1s state is considered here.
The binding energies for higher bound states where found to be lower than the minimum temperature found in the test cases here, thus they were assumed to be statistically not significant.
The ratio $\frac{g_{i+1}}{g_i}$ is $1/2$.
The number density of the states are related as $n_{i+1} = n_{H^+}= n_e^f =Z n_e$ and $n_i = n_H = n_e^b = n_e (1-Z)$.
The total electron number density is defined as $n_e = n_e^f + n_e^b$.
Thus, the IPD expression simplifies to
\begin{equation}
    \Delta_\text{IPD} = E_b - \mu + k_B T \ln{ \left[\frac{1}{2} \frac{1-Z}{Z} \right]}
    \,.
\end{equation}
An analytic fit for the chemical potential provided by \cite{Ichimaru_book_2018} is used here.
% Using the analytic expression for the chemical potential provided by \cite{Ichimaru_book_2018}

Outputs for dataset 3 are given in Fig. \ref{fig:optimized-outputs}.
As seen, the Rayleigh weight follows the behaviour observed above.
Some irregularities remain for the calculated IPD, I'm still figuring this one out.
Fig. \ref{fig:saha-output} gives an overview of the Saha equation output against the ionisation state $Z$ for all datasets considered.
As observed, it quickly diverges for values of the ionsation smaller than 0.2 or larger than 0.8.
This behaviour is shown to be bad for very high density, high temperature cases (i.e. $r_s = 1$, $\theta = 1$, and appears to worsen in particular with increasing temperature.
An alternative approach would be to use a similar model like the Stewart-Pyatt IPD model.
\textcolor{red}{The Saha ionization model is unable to correctly predict the behaviour of a hydrogen-like atom at high density, because it is based on exact energy levels of isolated ions and cannot take accurately model conditions where inter-atomic energies become dominant \cite{Larsen_2017}. \todo[inline]{Hannah: check this}
}

\begin{figure*}
    \includegraphics[width=\linewidth]{pics/old/variables_compared.png}
    \caption{Initial fitting outputs for dataset 3 ($r_s=3.23$) using the Saha equation to calculate IPD from the ionization state (optimisation variable).
    The cutoff for the calculated IPD is (0, -13.6).
    Left: calculated Rayleigh weight plotted against MCSS outputs against $q$.
    Right: optimized ionization (left axis)  and calculated IPD (right axis) against $q$.
    Some dependence on $q$ is observed.
    }
    \label{fig:optimized-outputs}
\end{figure*}

For the high temperature high density case, the ionization is shown to be around 1, which makes the IPD a bit of a useless variable to consider in the optimization process.
Outputs are basically useless at this point, so I need to have another look at that.
Similarly, for dataset 2 (mostly ionized plasma as well), results are not really indicative of anything (yet).

Fig. \ref{fig:surface-map-dataset3} shows the sensitivity of the fit to the ionisation.
For increasing $q$ (corresponding to larger scattering angles $\theta$), the sensitivity of the spectrum to the ionisation is significantly reduced.
Thus, the inelastic part of the spectrum is shown to be only sensitive to the ionisation for small scattering angles.



\begin{figure*}
    \includegraphics[width=\linewidth]{pics/old/Hannah_N14_rs3.23_theta1_surface_plot_log.png}
    \caption{Logarithmic surface plot of the error $\chi$ over $q-Z$ parameter space for dataset 3 [$r_s=3.23$].}
    \label{fig:surface-map-dataset3}
\end{figure*}

\begin{figure*}
    \includegraphics[width=\linewidth]{pics/old/Hannah_DATA_rs2_theta1_surface_plot_log.png}
    \caption{Logarithmic surface plot of the error $\chi$ over $q-Z$ parameter space for dataset 2 [$r_s=2$].}
    \label{fig:log-surface-map-dataset3}
\end{figure*}

% \begin{figure*}
%     \includegraphics[width=\linewidth]{pics/old/2_result_index=2_temperature_calculated.png}
%     \caption{
%     Representation of detailed balance for the MCSS structure factor outputs for dataset 2.
%     $q=1.40057$ is used here.
%     Left: The temperature calculated using detailed balance for each component of the structure factor from MCSS is plotted against $\omega$, the horizontal constants indicate the temperatures predicted by MCSS and Tobias' method.
%     Right: The free-free and bound-free structure factors are plotted for the negative scattering range.
%     }
% \end{figure*}

% \begin{figure*}
%     \includegraphics[width=\linewidth]{pics/old/3_result_index=9_temperature_calculated.png}
%     \caption{
%     Representation of detailed balance for the MCSS structure factor outputs for dataset 3 for $q=0.500693$.
%     Left: The temperature calculated using detailed balance for each component of the structure factor from MCSS is plotted against $\omega$, the horizontal constants indicate the temperatures predicted by MCSS and Tobias' method.
%     Right: The free-free and bound-free structure factors are plotted for the negative scattering range.
%     }
% \end{figure*}


\clearpage
\newpage

\subsection{Results for fit using the Saha equation input}

Results were re-run for a higher beam energy to ensure the q corresponds to a smaller angle and obtain a larger data set.

A quick test was performed to ensure probe energy did not influence the optimisation output as seen in Fig. \ref{fig:beam-energy-outputs}.
As seen, the beam energy chosen has virtually no impact on the resulting optimised values for the ionisation (and calculated ipd).
(Thank god for that...)
Ignoring outputs for higher-q (since previous results have shown there is little sensitivity to the ionisation at higher scattering angles), there is virtually no deviation based on the beam energy.
For these runs (and any following) an analytic source instrument function using a sharp Gaussian (with $\text{fwhm}=1\unit{eV}$) was used.

\begin{figure*}
    \includegraphics[width=\linewidth]{pics/old/fit_output_N32_rs3.23_theta1_compare_probe_energies.png}
    \caption{Outputs for $N=32$, $r_s=3.23$ and $\theta=1$ for a beam energy of 9000 and 20000 eV.}
    \label{fig:beam-energy-outputs}
\end{figure*}


\subsection{Best fit}

(Meaning fitting over all $q$ simultaneously.)
Notes:
\begin{itemize}
    \item Fitting results seem to be overly sensitive to higher $q$ values
    \item Filtering out the nan results from wrong angle calculations still gives weird results, i.e. very different best fit ionisation and ipd than using single points in $q$
\end{itemize}

Next steps:
\begin{itemize}
    \item Repeat fitting process, maybe pick datasets with $N=32$ to have more data points
    \item Consider weighing points to avoid overfitting for large $q$ where results are bullshit anyways, i.e. use a $1/q$ maybe somewhere (normalised)
    \item Repeat process for only the first few $q$-values to see if it works now
\end{itemize}


Update 30/096/2024

Chat with M. Bonitz at PNP18 pointed out some issues in the Saha equation treatment, he's provided a bit more context on the relationship between IPD, binding energy and continuum lowering.
His Master student is currently working on an analytical approach and will be sharing this equation with us, to replace the current Saha implementation with.


 \begin{figure*}
     \includegraphics[width=\linewidth]{pics/old/plot_SAVE.png}
     \caption{Initial best fit results plotted for dataset 3 $N=14$, $r_s=3.23$, $\theta=1$. Averaged chi plotted over all different ionisation values left and individual contributions for each $q$ plotted right.}
     \label{fig:best-fit-attempt-dataset3}
 \end{figure*}



 Next paper:
 - add MCMC simulator to see if we can get density and temperature to match
 


% \subsection{Updated results: 02.12.2024}

% Latest results are uploaded here, picked a few examples for each.

% \subsubsection{$N=14$, $r_s=2.5$, $\theta=1$}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/ionizations_error_N14_rs2.5_theta1.png}
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/N14_rs2.5_theta1_surface_plot_log.png}
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/N14_rs2.5_theta1_wr_surface_plot_log.png}
%     \caption{$N=14$, $r_s=2.5$, $\theta=1$ dataset. Top: ionisation error plot, arbitrarily normalised to enforce $f(Z=0)=1$. Middle: inelastic $\chi$-error over parameter space. Bottom: WR $\chi$-error surface plot.}
%     \label{fig:enter-label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/ionizations_error_N32_rs1_theta1.png}
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/N32_rs1_theta1_surface_plot_log.png}
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/N32_rs1_theta1_wr_surface_plot_log.png}
%     \caption{$N=32$, $r_s=1$, $\theta=1$ dataset. Top: ionisation error plot, arbitrarily normalised to enforce $f(Z=0)=1$. Middle: inelastic $\chi$-error over parameter space. Bottom: WR $\chi$-error surface plot.}
%     \label{fig:enter-label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/ionizations_error_N32_rs3.23_theta1.png}
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/N32_rs3.23_theta1_surface_plot_log.png}
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/N32_rs3.23_theta1_wr_surface_plot_log.png}
%     \caption{$N=32$, $r_s=3.23$, $\theta=1$ dataset. Top: ionisation error plot, arbitrarily normalised to enforce $f(Z=0)=1$. Middle: inelastic $\chi$-error over parameter space. Bottom: WR $\chi$-error surface plot.}
%     \label{fig:enter-label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/ionizations_error_N32_rs3.23_theta8.png}
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/N32_rs3.23_theta8_surface_plot_log.png}
%     \includegraphics[width=0.95\linewidth]{pics/old/results_02-12-2024/N32_rs3.23_theta8_wr_surface_plot_log.png}
%     \caption{$N=32$, $r_s=3.23$, $\theta=8$ dataset. Top: ionisation error plot, arbitrarily normalised to enforce $f(Z=0)=1$. Middle: inelastic $\chi$-error over parameter space. Bottom: WR $\chi$-error surface plot. \textcolor{red}{Check probe energy for middle panel.}}
%     \label{fig:enter-label}
% \end{figure}

